REST: Robust and Efficient Neural Networks for Sleep Monitoring in the Wild

In recent years, significant attention has been devoted towards integrating deep learning technologies in the healthcare domain. However, to safely and practically deploy deep learning models for home health monitoring, two significant challenges must be addressed: the models should be (1) robust against noise; and (2) compact and energy-efficient. We propose REST, a new method that simultaneously tackles both issues via 1) adversarial training and controlling the Lipschitz constant of the neural network through spectral regularization while 2) enabling neural network compression through sparsity regularization. We demonstrate that REST produces highly-robust and efficient models that substantially outperform the original full-sized models in the presence of noise. For the sleep staging task over single-channel electroencephalogram (EEG), the REST model achieves a macro-F1 score of 0.67 vs. 0.39 achieved by a state-of-the-art model in the presence of Gaussian noise while obtaining 19x parameter reduction and 15x MFLOPS reduction on two large, real-world EEG datasets. By deploying these models to an Android application on a smartphone, we quantitatively observe that REST allows models to achieve up to 17x energy reduction and 9x faster inference. We open-source the code repository with this paper: https://github.com/duggalrahul/REST.

==> Tables/comparison.tex <==
\begin{table}[!h]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{lrrr}
\toprule
\textbf{Method} & {\begin{tabular}[r]{@{}r@{}}\textbf{Macro-F1}\\ Benign / Noisy\end{tabular}} & \textbf{\begin{tabular}[r]{@{}r@{}}Params\\ ($\times 10^6$)\end{tabular}} & \textbf{\begin{tabular}[r]{@{}r@{}}Flops\\ ($\times 10^9$)\end{tabular}} \\ \hline
Sors & - & 2.26 & 1.45 \\
Biswal & - & 9.62 & 26.61 \\
Deep Residual & - & 18.62 & 6.49 \\
\method(sors) & - & - & - \\
\method(Biswal) & - & - & - \\
\method(Scott) & - & - & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Benchmark of recent SOTA \scott{what is SOTA?} models on the benign and gaussian noise corrupted sleep-EDF dataset.}
\label{tab:model_comparrson}
\end{table}

==> Tables/confusion-matrix.tex <==



\begin{table*}[t]
    \setlength{\tabcolsep}{9.2pt}
    % \small
    \centering
     \begin{tabular}{lcccccccc}  %lrrrrrrrr
     \toprule
     & \multicolumn{5}{c}{{\textbf{Predicted}}} & \multicolumn{3}{c}{{\textbf{Per-class Metrics}}} \\
     \cmidrule(l){2-6}\cmidrule(l){7-9}
     & W & N1  & N2  & N3 & REM & PR  & RE & F1  \\ 
    %  [0.5ex] 
     \midrule
    W & \textbf{1825 / 2345} & 26 / 71 & 58 / 44 & 0 / 1 & 127 / 136 & 0.98 / 0.93 & 0.70 / 0.90 & 0.82 / 0.91  \\
    N1 & 15 / 98 & \textbf{125 / 172} & 101 / 70 & 0 / 0 & 151 / 52 & 0.45 / 0.42 & 0.32 / 0.44 & 0.37 / 0.43  \\
    N2 & 16 / 54 & 22 / 85 & \textbf{3820 / 3812} & 161 / 94 & 89 / 63 & 0.83 / 0.85 & 0.93 / 0.93 & 0.88 / 0.89  \\
    N3 & 1 / 1 & 0 / 0 & 296 / 410 & \textbf{1128 / 1014} & 0 / 0 & 0.87 / 0.91 & 0.79 / 0.71 & 0.83 / 0.80  \\
    REM & 5 / 36 & 16 / 79 & 240 / 128 & 1 / 1 & \textbf{1342 / 1360} & 0.64 / 0.84 & 0.84 / 0.85 & 0.72 / 0.85  \\
    \bottomrule
    \end{tabular}
    \caption{Confusion matrix evaluating the performance of the \method-Sors$_C$(A+S) and benign trained Sors$_C$ model on the SHHS test dataset containing no noise. Our \method{} trained model is on the left, baseline right.}
    \label{tab:confusion-benign}
\end{table*}


\begin{table*}[t]
    % \setlength{\tabcolsep}{10pt}
    % \small
    \setlength{\tabcolsep}{10pt}
    \centering
     \begin{tabular}{lrrrrrrrr} 
     \toprule
     & \multicolumn{5}{c}{{\textbf{Predicted}}} & \multicolumn{3}{c}{{\textbf{Per-class Metrics}}} \\
     \cmidrule(l){2-6}\cmidrule(l){7-9}
     & W & N1  & N2  & N3 & REM & PR  & RE & F1  \\ 
    %  [0.5ex] 
     \midrule
    W & \textbf{2386 / 2564} & 26 / 4 & 58 / 29 & 0 & 127 / 0 & 0.93 / 0.63 & 0.92 / 0.99 & 0.92 / 0.77  \\
    N1 & 91 / 287 & \textbf{112 / 44} & 57 / 59 & 0 / 0 & 133 / 2 & 0.54 / 0.16 & 0.29 / 0.11 & 0.37 / 0.13  \\
    N2 & 43 / 357 & 44 / 42 & \textbf{3614 / 3686} & 165 / 22 & 242 / 1 & 0.89 / 0.70 & 0.88 / 0.90 & 0.89 / 0.79  \\
    N3 & 2 / 47 & 0 / 0 & 261 / 1003 & \textbf{1162 / 375} & 0 / 0 & 0.88 / 0.94 & 0.82 / 0.26 & 0.84 / 0.41  \\
    REM & 47 / 830 & 24 / 192 & 55 / 483 & 1 / 0 & \textbf{1477 / 99} & 0.75 / 0.97 & 0.92 / 0.06 & 0.82 / 0.12  \\
    \bottomrule
    \end{tabular}
    \caption{Confusion matrix evaluating the performance of the REST-Sors$_C$(A+S) model on the SHHS test dataset containing Gaussian noise at the medium level. Our \method{} trained model is on the left, baseline right.}
    \label{tab:confusion-guassian}
\end{table*}



